From dependent type theory to higher algebraic structures

The first part of this dissertation defines "dependently typed algebraic theories", which are a strict subclass of the generalised algebraic theories (GATs) of Cartmell. We characterise dependently typed algebraic theories as finitary monads on certain presheaf categories, generalising a well-known result due to Lawvere, B\'enabou and Linton for ordinary multisorted algebraic theories. We use this to recognise dependently typed algebraic theories for a number of classes of algebraic structures, such as small categories, n-categories, strict and weak omega-categories, planar coloured operads and opetopic sets. We then show that every locally finitely presentable category is the category of models of some dependently typed algebraic theory. Thus, with respect to their Set-models, these theories are just as expressive as GATs, essentially algebraic theories and finite limit sketches. However, dependently typed algebraic theories admit a good definition of homotopy-models in spaces, via a left Bousfield localisation of a global model structure on simplicial presheaves. Some cases, such as certain "idempotent opetopic theories", have a rigidification theorem relating homotopy-models and (strict) simplicial models. The second part of this dissertation concerns localisations of presentable $(\infty,1)$-categories. We give a definition of "pre-modulator", and show that every accessible orthogonal factorisation system on a presentable $(\infty,1)$-category can be generated from a pre-modulator by iterating a plus-construction resembling that of sheafification. We give definitions of "modulator" and "left-exact modulator", and prove that they correspond to those factorisation systems that are modalities and left-exact modalities respectively. Thus every left-exact localisation of an $\infty$-topos is obtained by iterating the plus-construction associated to a left-exact modulator.

==> chapters/homotopy-coherent-opetopic-algebras.tex <==
\chapter{Homotopy-coherent opetopic algebras}

We have seen that every category $\Oalg kn$ of opetopic algebras (such as the
categories $\Cat$, $\Opd\pl$ and $\Cmbd$ of small categories, coloured planar
operads and $PT$\=/combinads) can each be described as the category of models in
$\Set$ of an \emph{idempotent $\OO$-sorted theory}. Moreover, we have
characterised their fully faithful nerve functors to $\psh\OO$ by means of
projective sketches on the the category $\OO$ of opetopes.

In this short chapter, we will show that the nature of these sketches allows us
to use a general construction due to Horel (\cite{horel2015model}, generalised
in \cite{HorelCaviglia2016rigidification}) to obtain model structures on
$\s\Oalg kn$ (simplicial opetopic algebras) as well as on $\sPsh\bbLambda$
(simplicial presheaves on $\bbLambda$) that model what we will call
\emph{homotopy\=/coherent opetopic algebras}.

% \begin{remark}
%   I do not know whether homotopy\=/coherent opetopic algebras are a good notion
%   of 
% \end{remark}

We thus show that, at least for the categories $\Oalg kn$, there exist model
structures on their categories of simplicial objects that (ostensibly) model the
same structures up to homotopy. This can be seen as a very partial answer to the
general conjecture in~\cref{sec:htpical-models-C-cxl-cats}. 

\input{./chapters/homotopy-coherent-opetopic-algebras/homotopical-models}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> chapters/homotopy-models/gab-ulmer-loc.tex <==
\section{Background on Gabriel-Ulmer localisation}
\label{sec:backgr-gabr-ulmer-localisation}


% Let $C \in \Cat$, and let $\kappa \geq \omega$ be a regular cardinal. A
% morphism $f \in \psh C \arr$ is $\kappa$-small if and only if its domain and
% codomain are so. If $K$ is a set of $\kappa$-small morphisms of $\psh C$, then
% $C_K \subto \psh C$ preserves $\kappa$-filtered colimits. A category is
% \emph{locally $\kappa$-presentable} if and only if it is equivalent to one of
% the form $C_K$.

% The results of the previous paragraph still hold when $\psh\cC$ is replaced by
% a locally $\kappa$-presentable category.

% Let $\catDD$ be a locally presentable category, and let $K$ be a class of
% morphisms of $\catDD$. We say that $K$ is
% \emph{saturated}\footnote{``Abgeschlossen'' in \cite[paragraph
% 8.3]{Gabriel1971}.} if it contains all the isomorphisms of $\catDD$, is closed
% under colimits (in $\catDD\arr$), and satisfies ``2~out~of~3''. The smallest
% saturated class containing $K$ is called the \emph{saturation of $K$}. Assume
% now that $K$ is a \emph{set} rather than a class. Then ${}^\bot (\catDD_K)$ is
% the saturation of $K$, and the Gabriel--Ulmer localisation $a_K : \catDD \to
% \catDD_K \simeq K\inv \catDD$ of $\catDD$ at $K$ is also the localisation of
% $\catDD$ at ${}^\bot (\catDD_K)$.

% \subsubsection{Projective sketches}

% A \emph{projective sketch}\index{projective sketch} is the data of a $\cC \in
% \Cat$ and a set $K$ of cones in $\cC$. For $\catBB$ a category with all
% limits, the category of \emph{models in $\catBB$ of $(\cC, K)$} is the
% category of functors $\cC \to \catBB$ that take each cone in $K$ to a limit
% cone, and natural transformations between them. If $(\cC, K)$ is a projective
% sketch, then equivalently, $K$ can be seen as a set of cocones in $\cC^\op$,
% or as a set of sub-representables (subobjects of representables) in
% $\psh{\cC^\op}$. Let $\cC^\op _K \subto \psh{\cC^\op}$ be the full subcategory
% of all $X \in \psh{\cC^\op}$ such that $K \perp X$. Then $\cC^\op_K$ is
% precisely the category of models in $\Set$ of the projective sketch $(\cC,
% K)$. Let $\kappa$ be a regular cardinal, and let $(\cC, K)$ be a projective
% sketch in which each cone in $K$ is a $\kappa$-small diagram. Then $\cC^\op_K$
% is a locally $\kappa$-presentable category, and the inclusion $\cC^\op_K
% \subto \psh{\cC^\op}$ preserves $\kappa$-filtered colimits.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> chapters/opetopic-theories/dependently-sorted-species.tex <==
\section{The free-category monad}

Let $\bbtwo$ be the category with two~\cref{prop:loc-finite-finite-cover} objects $[0],[1]$ and two parallel
morphisms $s,t\colon [0] \to [1]$. $\psh\bbtwo$ is the category of (directed) graphs. Consider the
monad $T_\Cat\colon \psh\bbtwo \to \psh\bbtwo$ that takes a graph $X$ to the
underlying graph of its free category. Let $i : \Delta_0 \subset \psh\bbtwo$ be the
full subcategory of linear (or filiform) graphs of length $n \in \NN$.

By Weber \mytodo{cite}, $T_\Cat$ is the left Kan extension of $T_\Cat i$ along the
inclusion $i$. Now consider the wide, non-full subcategory $\Lambda_0$ of
$\Delta_0$ defined as follows:
\begin{align*}
  \relHom{\Lambda_0}{[m]}{[n]} &= \relHom{\Delta_0}{[m]}{[n]} \text{ if $m=0,1$},\\
                               &= \{*\} \text{ if $m=n$},\\
                               &= \emptyset \text{ otherwise.}
\end{align*}
Define the functor $F_\Cat : \Lambda_0 \to \psh\bbtwo$ as follows.
\[
  F_\Cat([0]) =
  \begin{tikzcd}
    \cdot \ar[loop]
  \end{tikzcd}\\
\]
\[
  F_\Cat([1]) = {\begin{tikzcd} \cdot \ar[loop] \ar[r] &\cdot \ar[loop]
    \end{tikzcd}}\\
\]
\[
  F_\Cat([n]) =
  \begin{tikzcd}
    \cdot \ar[loop] \ar[r]\ar[rrr,bend right] % &\ldots x_{n-1}\ar[loop] \ar[r]
     &\ldots\ar[r]&\cdot\ar[loop]\ar[r]&\cdot\ar[loop] 
   \end{tikzcd}
   \text{ ($n+1$ vertices)}.
\]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> chapters/small-obj-arguments/soa-wfs.tex <==
\section{Weak factorisation (after Quillen)}
\label{sec:weak-fact-quillen}
\begin{remark}
  [Adaptation to \oo\=/categories]
  \label{rem:quillen-adaptation-infty-cats} 
  Generalising the SOA for weak factorisation systems from $1$\=/categories to
  categories requires a small change. This is because the left class of a weak
  orthogonal system is stable under \emph{discrete} sums, but not under sums
  indexed by an arbitrary space (see \cref{rem:wos-defect-sum}). Thus, the SOA
  will require, for any pair of objects $A,B$ in a category $\cC$, a choice of
  cover $\relmap 0 A B \to \fun A B$ in $\cS$ from the set $\relmap 0AB$ of
  connected components of the mapping space $\fun AB$.
\end{remark}
\begin{para}
  We fix a small set of maps $W\to \cC\arr$ in a cocomplete category $\cC$. For
  any $f\colon X\to Y$ in $\cC$, we will describe a construction $\Quillenmap
  f$. Then the \emph{small object argument} will compute a factorisation of $f$
  for the weak orthogonal system $(\cA_W,\cB_W)$, by a transfinite iteration of
  the construction $\Quillenmap-$. First, remark that the condition $W\pitchfork
  f$ is equivalent to the existence of a diagonal lift in the single canonical
  square below (the fibre of $\pbh{\coprod_w\fun wf_0\times w}f$ over $\epsilon$
  is nonempty)
  % (namely, $\pbh{\coprod_w\fun wf_0\times w}f$ being a cover).
  \[
    \epsilon\ :\ \coprod_{w\in W} \fun w f _0 \times w\to f
  \]
  where $\fun{w}{f}_0$ is a chosen set of maps between $w$ and $f$ as
  in~\cref{rem:quillen-adaptation-infty-cats}, and $\fun w f _0 \times w =
  \coprod_{\fun w f _0} w$ is the usual tensor structure of $\cC\arr$ over $\cS$
  (the left-hand map above is thus a discrete coproduct of maps in $W$). The
  square defined by $\epsilon$ is
  \begin{equation}
    \tag{$\boxslash$}\label{eqn:liftcoend}
    \begin{tikzcd}[column sep=small]
      \coprod_{w} \fun w f _0 \times \s w \ar[r]\ar[d,"\coprod_w\fun{w}{f} \times w"']
      & \s f\ar[d, "f"]\\
      \coprod_{w} \fun w f _0 \times \t w \ar[r] & \t f.
    \end{tikzcd}
  \end{equation}
  We define the map $\Quillenmap f\colon \Quillen f\to \t f$ as the cocartesian
  gap map of this square.
  \begin{equation}
    \tag{$q$\=/construction}
    \label{eqn:qconstruction}
    \begin{tikzcd}[column sep=small]
      \coprod_{w} \fun w f _0\times \s w \ar[r]\ar[d,"\coprod_w\fun w f _0 \times w"']
      & \s f\ar[d,"u(f)"] \ar[ddr, bend left, "f"]&\\
      \coprod_{w} \fun w f _0\times \t w \ar[r, "\ell"'] \ar[rrd, bend right]
      & \Quillen f \ar[rd,"\Quillenmap f"'] \pomark &\\
      && \t f.
    \end{tikzcd}
  \end{equation}
  It is in fact more convenient to look at this as a diagram in $\cC\arr$:
  \begin{equation}
    \tag{$q$\=/lift}
    \label{eqn:qlift}
    \begin{tikzcd}[column sep=small]
      \coprod_{w} \fun w f _0\times \s w \ar[r]\ar[d,"\coprod_w\fun w f _0 \times w"']
      & \s f\ar[d, "f", near end] \ar[r, "u(f)"]
      & \Quillen f\ar[d, "\Quillenmap f"]\\
      \coprod_{w} \fun w f _0\times \t w \ar[r] \ar[rru, dashed, "\ell" near
      start]
      & \t f \ar[r,equal]
      & \t f.
    \end{tikzcd}
  \end{equation}
  Thus the map $\Quillenmap f$ can be understood as the best approximation of
  $f$ on the right that admits a lift from the map $\coprod_w\fun w f _0 \times
  w$.

  We thus obtain a factorisation of $f$ as $\Quillenmap fu(f)\colon \s f\to
  \Quillen f\to \t f$. The map $\coprod_w\fun w f _0 \times w$ is in $\cA_W$
  since $\cA_W$ is stable by discrete sums, and the map $u(f)\colon \s f\to
  \Quillen f$ is in $\cA_W$ since $\cA_W$ is stable by cobase change
  (\cref{lem:prop-wfs}). The map $\Quillenmap f\colon \Quillen f\to \t f$ need
  not be in $\cB_W$, but we will now show that it is so after a transfinite
  iteration.
\end{para}

\begin{theorem}[Small object argument]
  \label{thm:SOA}
  Let $\cC$ be a cocomplete category and let $W$ be a small set of arrows in
  $\cC$ with small domains. Then, the transfinite iteration of the
  $q$\=/construction converges to a factorization for the weak orthogonal system
  $(\cA_W, \cB_W)$ generated by $W$.
\end{theorem}

\begin{proof}
  The natural transformation $u\colon f\to \Quillenmap f$ defines a transfinite
  sequence
  \[
    f\xto{u(f)} \Quillenmap f\xto{u(\Quillenmap f)} \Quillenmapn2
    f\xto{u(\Quillenmapn2 f)} \dots
  \]
  We assumed that the domains $\s w$ were small for all $w\in W$. Let $\kappa$
  be a regular cardinals majoring the size of all $\s w$. The map $u^\kappa(f)$
  is in $\cA_W$ because it is a transfinite composite of maps in $\cA_W$
  (\cref{lem:prop-wos}). The result will be proven if we prove that the map
  $\Quillenmapn \kappa f $ is in $\cB_W=W^\pitchfork$.

  Let $w$ be in $W$, $\alpha:w\to \Quillenmapn \kappa f $ be a map and
  $L(\alpha)$ be its space of lifts. We wish to show that $L(\alpha)$ is not
  empty. We define $\Quillenn \kappa f\eqdef\s \Quillenmapn \kappa f$. Because
  $\s w$ is $\kappa$\=/small and $\kappa$ is $\kappa$\=/filtered, the map $\s
  w\to \Quillenn \kappa f $ associated to $\alpha$ factors through some
  $\Quillenn \lambda f $ for some ordinal $\lambda<\kappa$. By construction of
  $\Quillenn {\lambda+1} f $, we have a commutative diagram
\[
\begin{tikzcd}
\s w \ar[r]\ar[d, "w"'] 
& \Quillenn \lambda f \ar[d, "\Quillenmapn \lambda f "] \ar[rr, "u(\Quillenmapn \lambda f )"] 
&& \Quillenn {\lambda+1} f \ar[d, "\Quillenmapn {\lambda+1} f "]\ar[r]
&\dots \ar[r]
& \Quillenn \kappa f \ar[d, "\Quillenmapn \kappa f"]
\\
\t w \ar[r] \ar[rrru, dashed, bend left=10] 
& \t f \ar[rr, equal]
&& \t f \ar[r, equal] 
& \dots  \ar[r,equal] 
& \t f.
\end{tikzcd}
\]
and the dotted map provides the desired lift.
This finishes the proof that $f = \Quillenmapn \kappa f  u^\kappa(f)$ provides a factorisation of $f$ in $(\cA_W,\cB_W)$.
Moreover, the proof shows that this factorisation can be assumed natural in $f$.
\end{proof}



% \begin{rem}[A variant]
% \label{rem:Quillen-variant}
% When $\cC$ is a 1-category, the operator $W_Q(f) = \coprod_{w\in W} \fun w f _0
% \times w$ can be understood as the density comonad associated to the diagram $W\to \cC\arr$.
% \[
% \begin{tikzcd}
% W \ar[d] \ar[r] & \cC\arr \ar[loop right, "W_Q"]   \\
% \fun {W\op} \Set \ar[ru, dashed, "R", shift left] \ar[from=ru, dashed, "N", shift left]
% \end{tikzcd}
% \]
% The Quillen operator $q$ is then the pushout in the arrow category
% \[
% \begin{tikzcd}
% W_Q(f) \ar[r] \ar[d] & f \ar[d]
% \\
% \t_Q f \ar[r] & \Quillenmap f \pomark .
% \end{tikzcd}
% \]
% where $\t_Q f$ is the identity map of the codomain of $W_Q(f)$. 


% When $\cC$ is a general \oo category, the choice of set of morphisms of \ref{rem:quillen-adaptation-infty-cats} prevents such an interpretation.
% Nonetheless, it is possible to define a variant on Quillen's construction where we do not use such a set of maps, but the canonical space of maps.
% This variant supports the diagram $W\to \cC\arr$ to be indexed by an arbitrary category and not only a set.
% For such a diagram, we can define a density comonad $W_M$ 
% \[
% \begin{tikzcd}
% W \ar[d] \ar[r] & \cC\arr \ar[loop right, "W_M"]   \\
% \fun {W\op} \cS \ar[ru, dashed, "R", shift left] \ar[from=ru, dashed, "N", shift left]
% \end{tikzcd}
% \]
% and an operator $f\mapsto M(f)$
% \[
% \begin{tikzcd}
% W_M(f) \ar[r] \ar[d] & f \ar[d]
% \\
% \t_W f \ar[r] & M(f) \pomark .
% \end{tikzcd}
% \]
% where $\t_M f$ is the identity map of the codomain of $W(f)$. 
% The codomain of $M(f)$ is $\t f$ and thus $M(f)$ provides a factorization of $f$.
% Let $(\cA_W,\cB_W)$ be the WFS generated by $W$.
% The factorization of $f$ resulting from the iteration of $M$ has its right component in $\cB_W$.
% However, the left component is not in general in $\cA_W$:
% the map $W_M(f)= \colim_{W\comma F}w$ is a colimit of maps in $W$ but $\cA_W$ is not stable under colimits (since it would then be a FS). 
% This construction seems to provide a WFS between the WFS $(\cA_W,\cB_W)$ and the FS $(\cL_W,\cR_W)$.
% It is not clear to us what should be the extra property of such a WFS.
% Also, this setting seems related to the plus-construction, since the codomain of $W_M(f)$ is exactly the operator $\Plus f$ of \cref{defi:+construction}.
% \end{rem}


% \begin{rem}[Garner construction]
% \label{rem:garner1}
% Quillen's construction provides a pointed endofunctor $\pi_f\colon f \to \Quillenmap f$ on $\CC\arr$.
% In~\cite{Garner:SOA}, Garner establishes a variant on the construction by considering not the colimit of the sequence of $f \to \Quillenmap f\to \Quillenmapn2 f\to \dots$ but the free monad $\gamma$ generated by the pointed endofunctor $\pi:1\to q$.
% The map $\gamma(f)$ is essentially the quotient of $\Quillenmap f$ imposing that the two maps $q(\pi_f),\pi_{\Quillenmap f}:\Quillenmap f \to \Quillenmapn2 f$ coincide (as well as their analogs between higher iterations of $k$).
% The resulting map $\gamma(f)$ is still in the right class $\cR$ and is equipped with a free algebra structure over the pointed endofunctor $q$.
% The two constructions coincide if $\pi:1 \to q$ is a well-pointed endofunctor.
% \end{rem}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> tikz/common.tex <==
\usetikzlibrary{calc, decorations.pathmorphing, positioning}

% args: x, y, w, h, label, inner x, innner y
\newenvironment{TIKZZONE}[7]{
\begin{scope} [shift = {(#1, #2)}]
\draw [dotted] (0, 0) node [above right] {\small{\texttt{#5}}} -- (0, #4) -- (#3, #4) -- (#3, 0) -- cycle;
\begin{scope} [shift = {(#6, #7)}]
}{
\end{scope} \end{scope}
}

\tikzset{treeedge/.style = {above, sloped}}
\tikzset{treenode/.style = {circle, minimum size = 2pt, inner sep = 0, draw, fill}}

\newcommand{\blackwhitespoon}{-}
\newcommand{\DDownarrow}{|}
\newcommand{\optInt}[1]{\textbf{#1}}
\newcommand{\optOne}{\rightarrow}
\newcommand{\optZero}{\bullet}
\newcommand{\readdress}{P}
\newcommand{\RRightarrow}{-}
\newcommand{\Rrightarrow}{\equiv\!>}
\newcommand{\smalltriangleright}{>}
\newcommand{\src}{\mathsf{s}}
\newcommand{\system}{\textsc}
\newcommand{\tgt}{\mathsf{t}}
